Search and Society: Reimagining Information Access for Radical Futures

Information retrieval (IR) research must understand and contend with the social implications of the technology it produces. Instead of adopting a reactionary strategy of trying to mitigate potential social harms from emerging technologies, the community should aim to proactively set the research agenda for the kinds of systems we should build inspired by diverse explicitly stated sociotechnical imaginaries. The sociotechnical imaginaries that underpin the design and development of information access technologies needs to be explicitly articulated, and we need to develop theories of change in context of these diverse perspectives. Our guiding future imaginaries must be informed by other academic fields, such as human-computer interaction, information sciences, media studies, design, science and technology studies, social sciences, humanities, democratic theory, and critical theory, as well as legal and policy experts, civil rights and social justice activists, and artists, among others. In this perspective paper, we motivate why the community must consider this radical shift in how we do research and what we work on, and sketch a path forward towards this transformation.

==> 99-ack-arxiv.tex <==
\subsection*{Acknowledgements}
The author gratefully acknowledges feedback from Asia Biega, Michael D. Ekstrand, and Ida Larsen-Ledet on the various drafts of this paper.
